An Empirical Study of Dimensional Reduction Techniques for Facial Action Units Detection

Biologically inspired features, such as Gabor filters, result in very high dimensional measurement. Does reducing the dimensionality of the feature space afford advantages beyond computational efficiency? Do some approaches to dimensionality reduction (DR) yield improved action unit detection? To answer these questions, we compared DR approaches in two relatively large databases of spontaneous facial behavior (45 participants in total with over 2 minutes of FACS-coded video per participant). Facial features were tracked and aligned using active appearance models (AAM). SIFT and Gabor features were extracted from local facial regions. We compared linear (PCA and KPCA), manifold (LPP and LLE), supervised (LDA and KDA) and hybrid approaches (LSDA) to DR with respect to AU detection. For further comparison, a no-DR control condition was included as well. Linear support vector machine classifiers with independent train and test sets were used for AU detection. AU detection was quantified using area under the ROC curve and F1. Baseline results for PCA with Gabor features were comparable with previous research. With some notable exceptions, DR improved AU detection relative to no-DR. Locality embedding approaches proved vulnerable to \emph{out-of-sample} problems. Gradient-based SIFT lead to better AU detection than the filter-based Gabor features. For area under the curve, few differences were found between linear and other DR approaches. For F1, results were mixed. For both metrics, the pattern of results varied among action units. These findings suggest that action unit detection may be optimized by using specific DR for specific action units. PCA and LDA were the most efficient approaches; KDA was the least efficient.

==> experiments_old.tex <==
This section describes the experiments on RU-FACS \cite{bartlett2006automatic} and Spectrum \cite{cohn2009detecting} databases, which represent a more realistic AU detection scenario in terms of various races, ages, head movements, spontaneous expressions, and partial occlusions.
Our goal is to demonstrate in such diverse data which DR methods are beneficial for facial AU detection.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection {Datasets}
Two databases were used to investigate DR: RU-FACS  \cite{bartlett2006automatic} and Spectrum \citep{APA_1994}.  As explained in the next two sections, the observational scenario for both databases was an interview.  The databases differ in age of participants (older in Spectrum), head pose (near-frontal for RU-FACS and about 15 degrees from frontal for Spectrum), presence of psychopathology, and coding protocols.  For RU-FACS, only 'B' or higher intensity was coded; whereas all levels of intensity were coded for Spectrum.    
{\bf RU-FACS:}.  For these reasons, AU detection for Spectrum may be more challenging.

RU-FACS \cite{bartlett2006automatic} consists of video-recorded interviews of 100 young adults of varying ethnicity. Interviews were approximately two minutes in duration. Head pose was frontal with small to moderate out-of-plane rotation.  We had access to 34 of the interviews, of which video from five subjects could not be processed for technical reasons (e.g., noisy video). Thus, the experiments reported here were conducted with data from 29 participants. Metadata included manual FACS codes for AU onsets, peaks, and offsets. AU were coded if intensity was greater than "A" (i.e. trace, or lowest intensity on a 5-point scale).  Inter-observer agreement for FACS coding in RU-FACS has not been reported.  Because some AU occurred too infrequently, we selected the nine that occurred most frequently.   
%RU-FACS dataset \cite{bartlett2006automatic} is a large corpus of FACS coded interviews. Young adults were asked to either lie or tell the truth under a false opinion paradigm in interviews conducted by police and FBI members who posed around 13 questions. 
%These interviews resulted in 2.5 minute long continuous 30-fps video sequences containing spontaneous AUs of people of varying ethnicity and sex. 
%Ground truth FACS coding was provided by expert coders. 
%Data from 28 of the subjects was available for our experiments. 
%To make the results comparable, we followed \cite{zhu2011dynamic} and divided this dataset into 18 subjects for training ($\sim$97,000 frames) and the remaining for testing ($\sim$67,000 frames). 
%Previously published results on this dataset (\eg, [3]) are not directly comparable due to differences in the evaluation method; for comparison purposes, we implemented a frame-based Linear SVM.
 
{\bf Spectrum:}
Participants were 34 adults (67.6\% female, 88.2\% white, mean age 41.6 years) in the Spectrum database \citep{Cohn_2009} with a current diagnosis of major depressive disorder \citep{APA_1994} as determined using a structured clinical interview \citep{First_1995}. They were video-recorded during on one or more occasions at 7-week interviews during a semi-structured interview to assess depression severity (Hamilton Rating Scale for Depression, HRSD \citep{Hamilton_1967}. The interviews were recorded using four hardware-synchronized analogue cameras. Video from a camera roughly 15 degrees to the participant's right was digitized into 640x480 pixel arrays at a frame rate of 29.97 frames per second. 

Participant facial behavior was manually FACS coded from video by certified and experienced coders. AU onset, apex, and offset were coded for 17 commonly occurring AU. AU for all levels of intensity were coded (i.e. including 'A' or trace level intensity).  Overall inter-observer agreement for AU occurrence, quantified by CohenÕs Kappa was 0.75, which is considered a good reliability. The current study analyzed nine of these AU (Table I) that are conceptually related to affect and occurred frequently in the database (i.e., more than 5\% of the time).
%We selected the second dataset as the Spectrum database \cite{cohn2009detecting}, which comprises more complex appearance variations than RU-FACS.
%33 subjects (67.6\% females, 88.2\% Caucasian, and an average of 41.6 years) with major depressive disorder were interviewed to assess symptom severity over the course of treatment. 
%Interviews were recorded using four hardware-synchronized analogue cameras. 
%Image data from a camera approximately 15 degrees to the participant's right were used in the current study. 
%Video was digitized into 640$\times$480 pixel arrays with 24 bit resolution and a frame rate of 29.97 frames per second.
%As a result we filtered 69 sessions that contain valid tracking and FACS for evaluation.

%For both datasets, we selected the AUs of the most event occurrences to report our results, resulting in the AU list: $[1, 2, 4, 6, 10, 12, 14, 15, 17]$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection {Experimental Setup}

{\bf Tracking and alignment:}
Parameterized appearance models have been proven useful for facial feature alignment and face synthesis. 
In our study, we exploited the Active Appearance Models (AAMs) \cite{matthews2004active} that have been proven an excellent tool for aligning facial features with respect to a shape and appearance model. 
In particular, the AAM is composed of 66 facial landmarks that deform to fit perturbations in facial features (as illustrated in Fig.~\ref{fig:pipeline}(b)).
%Fig.~\ref{fig:pipeline}(b) shows the exampler tracked landmarks.

After tracking facial features using AAM, a similarity transform registers facial features with respect to a pre-computed average face (see Fig.~\ref{fig:pipeline}(c)). 
In the experiments reported here, the face was normalized into 200$\times$200 pixels.

\def\ft{We have done preliminary experiments on deciding the best scale for SIFT. Among 12$\times$12, 24$\times$24 and 36$\times$36 patches, we empirically chose the smallest scale since it gives the best overall accuracy.}

{\bf Appearance features:}
We explore the use of the SIFT descriptors and Gabor filter responses as appearance features following current success \cite{lucey2006aam,lucey2009automatically,tian2002evaluation}.
Since AUs happen only on subregions of the face, we extracted facial features only according to a subset of the 66 landmarks, \ie, 9 points for upper face and 7 points for lower face, as the red circles ({\color{red}{$\mathbf{\circ}$}}) depicted in Fig.~\ref{fig:pipeline}(d).
For all AUs, SIFT descriptors are built using a square of 12$\times$12 pixels\footnote{\ft}.
Gabor filter responses are computed as the output of four banks of 40 Gabor filters, comprising eight different orientations and five scales.
Each descriptor was then normalized into an unitary vector. 
%For each pixel within a subregion, SIFT descriptors add the pixel gradient vector to a histogram of gradient directions by quantizing each orientation to one of 8 directions and weighting the contribution of each vector by its magnitude.

{\bf Sample selection:}
Following previous work, positive samples were taken to be frames where the AU was present, and negative samples where it was not.
Since AU occurrence is relatively sparse among the entire video, we randomly downsampled to $\sim$20\% of the data with a 1:10 positive/negative ratio. 
Note that although better sampling strategies are possible (\eg, \cite{zhu2011dynamic}), in the experiments we observed comparable performance using DR techniques.

{\bf Evaluation metrics:}
To evaluate performance, we report two measures: Area Under the Curve (AUC) and the F1 score which is defined as $\text{F1} = \frac{2\cdot\emph{Recall}\cdot\emph{Precision}}{\emph{Recall} + \emph{Precision}}$.
The F1 summarizes the trade-off between high recall rates and accuracy among the predications. 
All measures were computed on a frame-by-frame basis by varying the bias or threshold of the corresponding classifier.
In our case, the F1 score is a better performance measure than the more common ROC metric because it is designed for balanced binary classification rather than detection tasks, and fails to reflect the effect of the proportion of positive to negative samples on classification performance.

\begin{table}
	\centering
	\footnotesize
	\begin{tabular}{@{}r|cccc}
		\toprule
		Methods & PCA & KPCA & LLE & LPP \\
		\midrule
		Time & 0.565s & 7.048s & 4.012s & 1.922s \\
		Computational & $\mathcal{O}(d^3)$ & $\mathcal{O}(n^3)$ & $\mathcal{O}(pn^2)$ & $\mathcal{O}(pn^2)$ \\
		Memory & $\mathcal{O}(d^2)$ & $\mathcal{O}(n^2)$ & $\mathcal{O}(pn^2)$ & $\mathcal{O}(pn^2)$ \\
		\midrule\midrule
		Methods & LDA & KDA & \multicolumn{1}{@{}c@{}|}{LSDA} & \\
		\cmidrule(r){1-4}
		Time &  0.594s & 19.029s & \multicolumn{1}{@{}c@{}|}{7.018s}  & \multicolumn{1}{l@{}}{$p: \#$neighbors} \\
		Computational & $\mathcal{O}(dnt+t^3)$ & $\mathcal{O}(n^3)$ & \multicolumn{1}{@{}c@{}|}{$\mathcal{O}(pn^2)$} & \multicolumn{1}{l@{}}{$t: \min(d,n)$}\\
		Memory & $\mathcal{O}(d^2)$ & $\mathcal{O}(n^2)$ & \multicolumn{1}{@{}c@{}|}{$\mathcal{O}(pn^2)$} & \\
	\bottomrule
	\end{tabular}
	\vspace{-1pt}\\
	%$^*$ The running time is reported on a subset of training data (details in text)
	\caption{Running time and complexities of DR techniques}
	\label{tab:complexity}
	\vspace{-24pt}
\end{table}
\input{tabRUFACS.tex}

{\bf Comparative methods:}
We implemented seven representative DR techniques by the following settings:
\begin{noindlist}
	\item[$\bullet$] PCA, KPCA, LPP: We kept 98\% energy for each method, resulting in $k=247,251,248$, respectively.
	\item[$\bullet$] LLE: We kept 98\% energy and set the number of neighbors $p=12$, resulting in $k = 258$. 
	\item[$\bullet$] LDA, KDA, LSDA: For supervised methods $k=1$, since AU detection is a binary problem, \ie, $\#\text{classes}=2$.
\end{noindlist}

{\bf Classifiers:}
In the experiments, we used linear SVM as the classifer \cite{holarge}. 
Parameter tuning was done using 5-fold subject-wise cross-validation on the training data. 
For all methods, we chose the parameters that maximize the averaged cross validation F1 score.

%In this procedure we first choose the feature that best predict (single) cross-validation performance and kept adding features until the cross-validation performance decreases with respect to a robust variation of F1.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection {Complexity and Computation Time}

Table \ref{tab:complexity} provides an overview into the running time, computational and memory complexities for each of the DR techniques.
These properties implies the applicability and feasibility to practical systems.
Though certain techniques are good at approximating the original source space, they are impractical to implement due to their high computational complexity.
For running time, we ran a sub-experiment on 300 positive and 3,000 negative samples and reported the results on the PC with CPU Intel i7 3.39GHz. 
The computational demand mostly lies on an eigen-decomposition process.
For kernel approaches, they involve an eigen-analysis of an $n\times n$ matrix and leads to the most computational time.

%%As the DR works in a high dimensional environment with large datasets, complexity of the reduction or clustering techniques is a major issue. 
%Hence for a term-document matrix, the complexity of DR varies based on the reduction technique used. 

  
%\subsection{Approximation Error}
\setlength{\ww}{.4\linewidth}
\begin{figure*}[t]
	\centering
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_RUFACS_AU1}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_RUFACS_AU2}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_RUFACS_AU4}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_RUFACS_AU6}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_RUFACS_AU10}\\
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_RUFACS_AU12}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_RUFACS_AU14}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_RUFACS_AU15}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_RUFACS_AU17}
	\vspace{-8pt}
	\caption{ROC curves on RU-FACS dataset using SIFT descriptors.}
	\label{fig:ROC:RUFACS:SIFT}
	\vspace{-8pt}
\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_RUFACS_AU1}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_RUFACS_AU2}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_RUFACS_AU4}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_RUFACS_AU6}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_RUFACS_AU10}\\
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_RUFACS_AU12}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_RUFACS_AU14}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_RUFACS_AU15}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_RUFACS_AU17}
	\vspace{-8pt}
	\caption{ROC curves on RU-FACS dataset using Gabor features.}
	\label{fig:ROC:RUFACS:Gabor}
	\vspace{-8pt}
\end{figure*}

\input{tabSpectrum.tex}
\begin{figure*}[t]
	\centering
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_Spectrum_AU1}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_Spectrum_AU2}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_Spectrum_AU4}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_Spectrum_AU6}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_Spectrum_AU10}\\
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_Spectrum_AU12}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_Spectrum_AU14}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_Spectrum_AU15}
	\includegraphics[width=\ww,trim=160 260 180 250]{sift_Spectrum_AU17}
	\vspace{-8pt}
	\caption{ROC curves on Spectrum dataset using SIFT features.}
	\label{fig:ROC:Spectrum:SIFT}
	\vspace{-8pt}
\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_Spectrum_AU1}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_Spectrum_AU2}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_Spectrum_AU4}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_Spectrum_AU6}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_Spectrum_AU10}\\
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_Spectrum_AU12}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_Spectrum_AU14}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_Spectrum_AU15}
	\includegraphics[width=\ww,trim=160 260 180 250]{gabor_Spectrum_AU17}
	\vspace{-8pt}
	\caption{ROC curves on Spectrum dataset using Gabor features.}
	\label{fig:ROC:Spectrum:Gabor}
	\vspace{-8pt}
\end{figure*}



\subsection{Results and Discussions}

We report our results on two appearance features and two datasets on Tables \ref{tab:RUFACS:sift} and \ref{tab:SPECTRUM:sift}.
To facilitate the comparison we illustrate the ROC curves for each AU in Figs.~\ref{fig:ROC:RUFACS:SIFT}$\sim$\ref{fig:ROC:Spectrum:Gabor}.
From the results obtained, we attempt to answer the following questions for the AU detection community:

\subsubsection{Lower-scale Gabor comparable with large-scale Gabor?}
\label{sec:disc:gabor}
%In this question we aim to contrast our results with previous findings on RU-FACS \cite{bartlett2006automatic}.
Our system computed the Gabor responses only on a small subset of facial landmarks (we called it \emph{low-scale} Gabor), and \cite{bartlett2006automatic} computed Gabor on entire face images (\emph{large-scale} Gabor) and did not apply feature selection.
Note that, following \cite{zhu2011dynamic}, we used 60\%/40\% for selecting training/testing subjects, while \cite{bartlett2006automatic} used leave-one-subject-out strategy and hence retained more information in the training phase.
Observe in Table \ref{tab:RUFACS:sift}(b), with appropriate DR, our results on AUs 1 and 2 are more consistent (AUs 1 and 2 are similar upper-face movements) and achieves $\sim$5\% higher AUC than \cite{bartlett2006automatic}.
However, our system performed $\sim$15\% worse in AU 4 and $\sim$5\% worse on average.
A possible explanation is because AU 4 concentrates only on the inner portion of the eyebrow but we fixed the facial landmarks for every upper face AU.
We argue that, with suitable DR technique and landmark selection for different AUs, lower-scale Gabor can provide more reasonable results with greater efficiency.

%The reason is that local appearance features are typically invariant to illumination changes and deformations.

\subsubsection{A better appearance representation?}
Following the settings on RU-FACS \cite{zhu2011dynamic}, we are able to replicate similar results, ensuring that our systems worked in a reasonable manner.
Observe from Tables \ref{tab:RUFACS:sift} and \ref{tab:SPECTRUM:sift}, gradient-based SIFT consistently outperforms filter-based Gabor features across AUs and DR techniques, which has also been shown in \cite{zhu2011dynamic}.
This is because SIFT considers histograms of gradient orientations that potentially capture much FACS information such as naso-labial furrows and slope of eyebrows, and thus achieves the robustness to illumination changes and small errors in localization.
Moreover, we found that with proper DR techniques, the system achieved comparable performance within $\sim$2\% AUC on average.
As a result, we converge to the conclusion that gradient-based SIFT leads to better AU detection than the filter-based Gabor features.

\subsubsection{DR affords advantages beyond efficiency?}
Despite the needs for DR (as mentioned in Sec.~\ref{sec:intro}), we explored further the benefits of DR approaches by including a no-DR control condition in the experiments.
Surprisingly, in Table \ref{tab:RUFACS:sift}, DR approaches generally improve not only the computational efficiency but also the performance.
\vincent{Harry could you check the no-DR number for RU-FACS?}

\subsubsection{Which DR yield improved AU detection?}
In the study we compared four types of DR techniques including linear, manifold, supervised and hybrid.
There is not an overall winner across these types but we make the interesting observations:
(a) Kernel extensions do not always perform better.
Instead, in our experiments, PCA/LDA usually outperforms KPCA/KDA.
This can be explained by the \emph{curse of dimensionality} as the number of data grows exponentially with the dimensions in the subspace.
Lifting the data to high-dimensional feature space requires construction of a proper kernel which leads to high computational costs.
Moreover, selection of parameters can be another issue, \eg, too small $\sigma$ for RBF kernel results in overfitting and large $\sigma$ introduces sensitivity to outliers.
(b) Manifold methods, considering neighborhood relationships, do not necessarily reflect the global AU structure.
The smoothness assumption of manifolds limits the modelling in the presence of noise and discontinuities in manifolds.
Data points face the difficulty to find good neighbors when the sampling space is too sparse. 
This is usually the case in AU detection since it is hard to represent the entire AU space with all possible face variations.
The poor performance of LLE in our experiments support this claims.
On the other hand, LPP is defined to cover the ambient space rather than just on the training samples (such as LLE), and thus can avoid the out-of-sample problem. 
%Compared with PCA, LPP concerns the locally distance with neighbors. 
%Hence, it requires that the number of AU frames should be relatively large enough in order to find good enough neighbors. 
Observed from the experiments, the AUs with lots of samples can render good performance by using LPP, such as AU 12 on RU-FACS, and AU 14 on Spectrum.
(c) Supervised methods generally help improve 3$\sim$6\% in AUC and up to 8\% in F1, as label information provides more discriminative properties for calculating the embedding.
%As one can observe that the performance of LLE on both datasets are quite unsatisfactory.

%LLE performs worse than the other DR approaches as it is likely to confront with manifolds that contains holes, \ie, the out-of-sample problem.

%(2) LDA can perform well when the number of data points are greatly larger than the dimension of features, which has been illustrated in the previous section. Observe the results on Spectrum, compared SIFT+LDA with Gabor+LDA, the performance of AU12 increases a lot with the Gabor feature. One possible explanation is because the dimension of Gabor feature ($d$=240) is smaller than the dimension of SIFT ($d$=768), and thus the frames of AU12 can be much larger than the dimension of Gabor.  On the other hand, for AU14, the number of labeled frames is already very large and the change of dimension of feature does not make much difference.
%\vincent{Need double check this}

%(3) KPCA mainly focuses on large pairwise distance, however, it is not suitable to characterize facial AUs, which may be tiny changes in distance and thus other condition rather than facial action unit may be captured.

%(4) Compared with LLE, LPP is defined everywhere in ambient space rather than just on the training data points and thus can overcome the out of sample problem. Compared with PCA, LPP concerns the locally distance with neighbors. Hence, it requires that the number of AU frames should be relatively large enough in order to find good enough neighbors. Observed from the experiments, the AUs with lots of samples can render good performance by using LPP, such as AU12 in RUFACS, and AU14 in Spectrum.

%(5) A subset of AUs appear more ``linear'' than others.  For instance, when applying PCA/LDA on AUs 1, 2,


%We hope to see:
%\begin{itemize}
%	\item Linear/nonlinear approaches are able to capture the properties of ``conceptually'' linear/nonlinear AUs.
%	\item DR are comparable with No-DR in terms of accuracy, while using much fewer dimensions than the input data (more efficient?).
%	\item DR can sometimes outperform No-DR because outliers/noise are removed?
%	\item SIFT can perform better than Gabor.
%	\item Locally embedded approaches do not really help AU detection tasks, as the nearest neighbor assumption does not hold in a testing dataset.
%\end{itemize}


==> tabSpectrum.tex <==
\begin{table*}
	\centering
	(A) 
	\begin{tabular}{@{\ }c@{\ }||@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }}
		\toprule
		SIFT & \multicolumn{8}{@{\ }c|@{\ }}{Area Under Curve} & \multicolumn{8}{@{\ }c@{\ }}{F1 Score}\\ 
		\cmidrule{2-9}\cmidrule{10-17}
		{\bf Type} & --- & \multicolumn{2}{@{\ }c|@{\ }}{Linear} & \multicolumn{2}{@{\ }c|@{\ }}{Manifold} & \multicolumn{1}{@{\ }c|@{\ }}{Hybrid} & \multicolumn{2}{@{\ }c|@{\ }}{Supervised}
			& --- & \multicolumn{2}{@{\ }c|@{\ }}{Linear} & \multicolumn{2}{@{\ }c|@{\ }}{Manifold} & \multicolumn{1}{@{\ }c|@{\ }}{Hybrid} & \multicolumn{2}{@{\ }c@{\ }}{Supervised} \\
		\midrule
		\bf{AU} & {\bf{No-DR}} & {\bf{PCA}} & {\bf{KPCA}} & {\bf{LPP}} & {\bf{LLE}} & {\bf{LSDA}} & {\bf{LDA}} & {\bf{KDA}} 
		        & {\bf{No-DR}} & {\bf{PCA}} & {\bf{KPCA}} & {\bf{LPP}} & {\bf{LLE}} & {\bf{LSDA}} & {\bf{LDA}} & {\bf{KDA}}\\
		\midrule
		1	 & .69 &.58 &.58&.51 & .38&.58 &.68 &.66 &  .28& .24 & .23 & .20 & .21 & .23 & .30 & .29\\
		2	 & .72 &.67 &.58&.62 & .50&.71 &.70 &.69 &  .32& .31 & .21 & .23 & .19 & .29 & .31 & .27\\
		4	 & .67 &.69 &.74&.65 & .60&.67 &.70 &.76 &  .35& .38 & .45 & .37 & .27 & .34 & .39 & .48 \\
		6	 & .70 &.68 &.66&.71 & .46&.74 &.70 &.81 &  .22& .21 & .19 & .22 & .14 & .24 & .22 & .34 \\
		10 & .68 &.54 &.51&.44 & .44&.51 &.64 &.66 &  .43& .39 & .36 & .36 & .35 & .36 & .43 & .44 \\
		12 & .80 &.79 &.80&.79 & .74&.57 &.73 &.75 &  .60& .55 & .57 & .56 & .52 & .37 & .48 & .57 \\
		14 & .82 &.83 &.85&.84 & .67&.77 &.83 &.74 &  .58& .62 & .62 & .64 & .46 & .63 & .65 & .54 \\
		15 & .59 &.64 &.56&.52 & .52&.67 &.66 &.55 &  .18& .23 & .10 & .10 & .08 & .16 & .15 & .08 \\
		17 & .52 &.50 &.50&.43 & .55&.50 &.49 &.58 &  .38& .38 & .38 & .38 & .39 & .37 & .38 & .39\\ \midrule
		Avg& .69 &.66 &.64&.61 & .54&.64 &.68 &.69 &  .37& .37 & .35 & .34 & .29 & .33 & .37 & .38 \\
		\bottomrule
	\end{tabular}
	\vspace{10pt}
	
	(B)
	\begin{tabular}{@{\ }c@{\ }||@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }|@{\ }c@{\ }|@{\ }c@{\ }@{\ }c@{\ }}
		\toprule
		Gabor & \multicolumn{8}{@{\ }c|@{\ }}{Area Under Curve} & \multicolumn{8}{@{\ }c@{\ }}{F1 Score}\\ 
		\cmidrule{2-9}\cmidrule{10-17}
		{\bf Type} & --- & \multicolumn{2}{@{\ }c|@{\ }}{Linear} & \multicolumn{2}{@{\ }c|@{\ }}{Manifold} & \multicolumn{1}{@{\ }c|@{\ }}{Hybrid} & \multicolumn{2}{@{\ }c|@{\ }}{Supervised}
			& --- & \multicolumn{2}{@{\ }c|@{\ }}{Linear} & \multicolumn{2}{@{\ }c|@{\ }}{Manifold} & \multicolumn{1}{@{\ }c|@{\ }}{Hybrid} & \multicolumn{2}{@{\ }c@{\ }}{Supervised} \\
		\midrule
		\bf{AU} & {\bf{No-DR}} & {\bf{PCA}} & {\bf{KPCA}} & {\bf{LPP}} & {\bf{LLE}} & {\bf{LSDA}} & {\bf{LDA}} & {\bf{KDA}} 
		        & {\bf{No-DR}} & {\bf{PCA}} & {\bf{KPCA}} & {\bf{LPP}} & {\bf{LLE}} & {\bf{LSDA}} & {\bf{LDA}} & {\bf{KDA}}\\
		\midrule
		1	 & .73 &.53 &.52&.68 & .42&.61 &.67 & .52 &  .29& .21 & .22 & .30 & .21 & .25 & .30 & .22 \\
		2	 & .81 &.56 &.70&.63 & .50&.73 &.70 & .65 &  .57& .20 & .31 & .24 & .19 & .33 & .27 & .27 \\
		4	 & .82 &.81 &.81&.68 & .64&.73 &.79 & .52 &  .56& .51 & .45 & .34 & .33 & .42 & .49 & .25 \\
		6	 & .68 &.62 &.48&.60 & .47&.70 &.72 & .63 &  .20& .17 & .14 & .17 & .13 & .23 & .25 & .18 \\
		10 & .67 &.61 &.40&.53 & .48&.63 &.67 & .51 &  .42& .39 & .35 & .35 & .35 & .41 & .43 & .35 \\
		12 & .81 &.74 &.71&.74 & .58&.84 &.83 & .72 &  .57& .48 & .47 & .50 & .41 & .58 & .58 & .48 \\
		14 & .81 &.86 &.76&.83 & .49&.83 &.83 & .66 &  .58& .70 & .55 & .64 & .40 & .63 & .61 & .46 \\
		15 & .39 &.38 &.40&.41 & .58&.43 &.46 & .55 &  .07& .07 & .07 & .07 & .09 & .07 & .07 & .09 \\
		17 & .52 &.54 &.43&.54 & .49&.50 &.53 & .52 &  .38& .38 & .38 & .38 & .38 & .38 & .38 & .38 \\ \midrule
		Avg& .69 &.63 &.58&.63 & .53&.67 &.69 & .59 &  .40& .35 & .33 & .33 & .28 & .37 & .38 & .30 \\
		\bottomrule
	\end{tabular}
	
	\vspace{-1pt}
	\caption{Performance on the SPECTRUM dataset using (a) SIFT and (b) Gabor features.}
	\label{tab:SPECTRUM:sift}
	\vspace{-10pt}
\end{table*}


